Possibility results for graph clustering: A novel consistency axiom

Kleinberg introduced three natural clustering properties, or axioms, and showed they cannot be simultaneously satisfied by any clustering algorithm. We present a new clustering property, Monotonic Consistency, which avoids the well-known problematic behaviour of Kleinberg's Consistency axiom, and the impossibility result. Namely, we describe a clustering algorithm, Morse Clustering, inspired by Morse Theory in Differential Topology, which satisfies Kleinberg's original axioms with Consistency replaced by Monotonic Consistency. Morse clustering uncovers the underlying flow structure on a set or graph and returns a partition into trees representing basins of attraction of critical vertices. We also generalise Kleinberg's axiomatic approach to sparse graphs, showing an impossibility result for Consistency, and a possibility result for Monotonic Consistency and Morse clustering.

==> intro.tex <==

\usepackage{setspace}
\doublespacing

\usepackage{amsmath, amsfonts,amssymb}
\usepackage{multicol}
\usepackage{color}
\usepackage{xspace}
\usepackage{enumerate}

\usepackage{appendix}
\usepackage{pifont}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{float}
\usepackage{tcolorbox}
\usetikzlibrary{decorations.markings}
\graphicspath{ {images/} }
\usepackage{arydshln}
\usepackage[algo2e,boxed]{algorithm2e}
\usepackage{hyperref}
\hypersetup{pdfauthor=author}
\usepackage{cleveref}
\usepackage{natbib}
\bibliographystyle{elsarticle-num-names}

\newcommand{\then}{\ensuremath{\Rightarrow}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Morse}{\texttt{Morse}~}
\newcommand{\comm}[1]{}
\renewcommand{\Phi}{\varPhi}
\renewcommand{\phi}{\varphi}
\newcommand{\xmark}{\ding{55}}
\hfuzz=20pt
\vfuzz=20pt
\hbadness=2000
\vbadness=\maxdimen

\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma} 
\newtheorem{proposition}[theorem]{Proposition} 
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}

\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox}%\\[2mm]}


\long\def\acks#1{\vskip 0.3in\noindent{\large\bf Acknowledgments}\vskip 0.2in
\noindent #1}

